CPR: Retrieval Augmented Generation for Copyright Protection

Retrieval Augmented Generation (RAG) is emerging as a flexible and robust technique to adapt models to private users data without training, to handle credit attribution, and to allow efficient machine unlearning at scale. However, RAG techniques for image generation may lead to parts of the retrieved samples being copied in the model's output. To reduce risks of leaking private information contained in the retrieved set, we introduce Copy-Protected generation with Retrieval (CPR), a new method for RAG with strong copyright protection guarantees in a mixed-private setting for diffusion models.CPR allows to condition the output of diffusion models on a set of retrieved images, while also guaranteeing that unique identifiable information about those example is not exposed in the generated outputs. In particular, it does so by sampling from a mixture of public (safe) distribution and private (user) distribution by merging their diffusion scores at inference. We prove that CPR satisfies Near Access Freeness (NAF) which bounds the amount of information an attacker may be able to extract from the generated images. We provide two algorithms for copyright protection, CPR-KL and CPR-Choose. Unlike previously proposed rejection-sampling-based NAF methods, our methods enable efficient copyright-protected sampling with a single run of backward diffusion. We show that our method can be applied to any pre-trained conditional diffusion model, such as Stable Diffusion or unCLIP. In particular, we empirically show that applying CPR on top of unCLIP improves quality and text-to-image alignment of the generated results (81.4 to 83.17 on TIFA benchmark), while enabling credit attribution, copy-right protection, and deterministic, constant time, unlearning.

==> supp_matt.tex <==
\input{preamble}

\begin{proof} of \cref{prop:mixture-of-score}.
\begin{align}
\nabla_{x_t} \log p_t(x_t|c) &=  \nabla_{x_t} \log \int p_t(x_t|x_0)\big[w_0p_D(x_0|c) + w_1p_{D_\text{retr}}(x_0|c)\big]dx_0 \nonumber \\
&= \dfrac{1}{\int p_t(x_t|x_0)\big[w_0p_D(x_0|c) + w_1p_{D_\text{retr}}(x_0|c)\big]dx_0} \Big[\nabla_{x_t} \int p_t(x_t|x_0) w_0p_D(x_0|c) dx_0 \nonumber \\ &+  \nabla_{x_t} \int p_t(x_t|x_0) w_1p_{D_\text{retr}}(x_0|c) dx_0\Big] \nonumber \\
&= \dfrac{1}{p_t(x_t|c)} \Big[\nabla_{x_t} \int p_t(x_t|x_0) w_0p_D(x_0|c) dx_0 +  \nabla_{x_t} \int p_t(x_t|x_0) w_1p_{D_\text{retr}}(x_0|c) dx_0\Big] \nonumber \\
&= \dfrac{1}{p_t(x_t|c)} \Big[w_0\int p_t(x_t|x_0) p_D(x_0|c) dx_0 \nabla_{x_t} \log \int p_t(x_t|x_0) p_D(x_0|c) dx_0 \nonumber \\ &+  w_1\int p_t(x_t|x_0) p_{D_\text{retr}}(x_0|c) dx_0 \nabla_{x_t} \log \int p_t(x_t|x_0) p_{D_\text{retr}}(x_0|c) dx_0\Big] \nonumber \\
&= \dfrac{w_0\int p_t(x_t|x_0) p_D(x_0|c) dx_0}{p_t(x_t|c)} \nabla_{x_t} \log \int p_t(x_t|x_0) p_D(x_0|c) dx_0 \nonumber \\ &+  \dfrac{w_1\int p_t(x_t|x_0) p_{D_\text{retr}}(x_0|c) dx_0}{p_t(x_t|c)}  \nabla_{x_t} \log \int p_t(x_t|x_0) p_{D_\text{retr}}(x_0|c) dx_0\ \nonumber
\end{align}
\end{proof}

\begin{proof} of \cref{prop:prompt}.
Let $s_{\theta_1}(x_t, t, c) \triangleq s_{\theta_0 + \Delta \theta_1}(x_t, t, c)$ be the optimal solution to the retrieval optimization problem. We use $\operatorname{CLIP}$ embeddings of the retrieved images for generation, and bound its difference from the optimal.
\begin{align}
\|s_{\theta_1}(x_t, t, c)-\hat{s}_{\theta_0}(x_t, t, c_{\text{test}})\| &=
\|s_{\theta_1}(x_t, t, c)-s_{\theta_0}\Big(x_t, t, \frac{1}{m} \sum_{x_i \in \Dr}\text{CLIP}(x_i)\Big)\| \nonumber \\
&= \|s_{\theta_1}(x_t, t, c) - s_{\theta_0}(x_t, t, c) + s_{\theta_0}(x_t, t, c) -  s_{\theta_0}\Big(x_t, t, \frac{1}{m} \sum_{x_i \in \Dr}\text{CLIP}(x_i)\Big)\| \nonumber \\
&\leq \|s_{\theta_1}(x_t, t, c) - s_{\theta_0}(x_t, t, c)\| + \|s_{\theta_0}(x_t, t, c) -  s_{\theta_0}\Big(x_t, t, \frac{1}{m} \sum_{x_i \in \Dr}\text{CLIP}(x_i)\Big)\| \nonumber \\
&\leq \|s_{\theta_0 + \Delta \theta_1}(x_t, t, c) - s_{\theta_0}(x_t, t, c)\| + \|s_{\theta_0}(x_t, t, c) -  s_{\theta_0}\Big(x_t, t, \frac{1}{m} \sum_{x_i \in \Dr}\text{CLIP}(x_i)\Big)\| \nonumber \\
&\leq l_{\theta} \|\Delta \theta_1\| + l_{c} \|\frac{1}{m} \sum_{x_i \in \Dr}\text{CLIP}(x_i)\|
\end{align}
\end{proof}

\begin{proof} of \cref{lemma:cpr-kl}. \cite{vyas2023provable} proved in Theorem 3.1, that sampling from \cref{eq:prod-sampling} produces samples which are copy-protected. We need to show that using Langevin based backward diffusion in \cref{algo:cpr-kl} indeed generates samples from the desired distribution. Towards this, we will use the results from \cite{yang2022convergence}. More precisely, assuming that the target distribution in \cref{eq:prod-sampling} satisfies, Assumption 1-4 in Section 3 \cite{yang2022convergence} (it satisfies Log-Sobolev inequality, the true score is lipschitz, the score estimator is lipschitz, and the error of the score estimator has a finite moment generating function), then \cite{yang2022convergence} showed in Corollary 1 that KL-divergence between the distribution sampled using \cref{algo:cpr-kl} and \cref{eq:prod-sampling} approaches 0, as $T,N \rightarrow \infty$ and $\epsilon_t \rightarrow 0$.
\end{proof}

{\small
\bibliography{supp_matt}}
